Chronological Causal Bandits

This paper studies an instance of the multi-armed bandit (MAB) problem, specifically where several causal MABs operate chronologically in the same dynamical system. Practically the reward distribution of each bandit is governed by the same non-trivial dependence structure, which is a dynamic causal model. Dynamic because we allow for each causal MAB to depend on the preceding MAB and in doing so are able to transfer information between agents. Our contribution, the Chronological Causal Bandit (CCB), is useful in discrete decision-making settings where the causal effects are changing across time and can be informed by earlier interventions in the same system. In this paper, we present some early findings of the CCB as demonstrated on a toy problem.

==> figures/fig_sections/__latexindent_temp.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}{.35\textwidth}
      \centering
      \includegraphics[width=1.\linewidth]{figures/CR_scmmab.pdf}
      \caption{\scmmab at $t=1$. \label{fig:t1_SCMMAB}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{.35\textwidth}
      \centering
      \includegraphics[width=1.\linewidth]{figures/CR_ccb.pdf}
      \caption{\ccb at $t=1$\label{fig:t1_CCB}}
    \end{subfigure}%
    \caption{CR
    \label{fig:results}}
\end{figure}


==> figures/fig_sections/fig_notation_plot.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/notation_plot.eps}
    \caption{Unrolling}
    \label{fig:notation_plot}
\end{figure*}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/alg.tex <==
\begin{figure}
\begin{minipage}{.55\textwidth}
 \scalebox{0.90}{
\begin{algorithm}[H]
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\KwData{$\dataset^O$, $\{\DIntXstzero\}_{s \in \{0,\dots, |\missets_0|\}}$, $\graph_{0:T}$, 
	$P$. }
	\KwResult{Optimal intervention path $\{\Xst^\star, \xst^\star, y_t^\star\}_{t = 1}^T$}
	\textbf{Initialise}: $\missets$, $\dataset^I_0$ and initial optimal $\DIopt = \emptyset$.\\
	\For{$t = 0, \dots, T$}{ 
	1. Initialise dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\mathcal{D}^I_{\star,t-1}$ if $t>0$. \\
	2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$ \\
	\For{$p = 1, \dots, P$}{
	1. Compute $\EIst(\x)$ for each $\Xst \in \missets_t$.\\
	2. Obtain $(s^\star, \alpha^\star)$ \\
	3. Intervene and augment $\DIntXsstar$ \\
	4. Update posterior for $f_{s=s^\star, t}$
    }
    3. Return the optimal intervention $(\Xst^\star, \xst^\star)$\\
    4. Append optimal interventional data $\mathcal{D}^I_{\star,t} = \mathcal{D}^I_{\star,t-1} \cup ((\Xst^\star, \xst^\star), y^\star_t)$
	}
	\caption{\our}
	\label{alg:dcbo_alg}
\end{algorithm}
}
\end{minipage}

\begin{minipage}{.45\textwidth}



% \includegraphics[width=0.9\linewidth]{figures/graphs_vertical.eps}
% \caption{\DAG{s} used in the experimental sessions for the real and synthetic data.}
% \label{fig:dag_experiments}

\input{figures/experimental_dags}


\end{minipage}
\end{figure}

% \begin{algorithm}[t]
% 	\SetKwInOut{Input}{input}
% 	\SetKwInOut{Output}{output}
% 	\KwData{$\dataset^O$, $\{\DIntXstzero\}_{s \in \{0,\dots, |\missets_0|\}}$, $\graph_{0:T}$, 
% 	$P$. }
% 	\KwResult{Optimal intervention path $\{\Xst^\star, \xst^\star, y_t^\star\}_{t = 1}^T$}
% 	\textbf{Initialise}: $\missets$, $\dataset^I_0$ and initial optimal $\DIopt = \emptyset$.

% 	\For{t = 0, \dots, T}{\\ 
% 	1. Initialize dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\DIopt_{t-1}$ if $t>0$. \\
% 	2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$ \\
% 	\For{p = 1, \dots, P}{
% 	1. Compute $\EIst(\x)$ for each $\Xst \in \missets_t$.\\
% 	2. Obtain $(s^\star, \alpha^\star)$.\\
% 	3. Intervene and augment $\DIntXsstar$.\\
% 	4. Update posterior for $f_{s=s^\star, t}$
%     }
%     3. Return the optimal intervention $(\Xst^\star, \xst^\star)$.\\
%     4. Append optimal interventional data $\DIopt_t = \DIopt_{t-1} \cup ((\Xst^\star, \xst^\star), y^\star_t)$.
% 	}
% 	\caption{Dynamic Causal Bayesian Optimisation (\our)}
% 	\label{alg:dcbo_alg}
% \end{algorithm}

% 	Compute $\epsilon$ and sample $u \sim \mathcal{U}(0, 1)$.
% 	\If{$\epsilon > u$}{(Observe) \\
% 	1. Collect new observations $\mat{v}_t$. \\
% 	2. Augment $\dataset^O_t = \observations \cup \{\mat{v}_t\}$.\\
% 	3. Update prior surrogate models. 
% 	}
% 	\Else{(Intervene)\\
	%\; 1. Initialize dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\DIopt_{t-1}$ if $t>0$.
	%2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$.

==> sections/connections_old.tex <==
\subsection{Connections}

The problem setup we study differs from those considered by both \cbo \cite{cbo} and \abo \cite{abo}. In this section we draw the links between these methods highlighting the reasons why \our is needed to solve the problem in \eq \eqref{eq:dcgo}. See \fig \ref{fig:map_methods} for a graphical representation of the relationship between \our and alternative optimization methods. A thorough discussion is included in the appendix (\S X).

\textbf{\cbo algorithm} \cbo tackles the causal dimension of the \dgo problem but not the temporal dimension. While it can be used to find optimal interventions to perform in a \DAG, this algorithm addresses static settings where variables in $\graph$ are i.i.d. across time steps, \ie $p(\mat{V}_t) = p(\mat{V})\text{,}\forall t$, and only one static target variable exists. For instance, \cbo can be used to find the optimal intervention for $Y$ in \fig \ref{fig:map_methods}, plate (b). Finding an optimal sequence of interventions for the \DAG in \fig \ref{fig:map_methods} plate (d) requires running \cbo for $T$ times optimizing $\Yt$ at each time step. In doing that \cbo re-initializes all surrogate models at every $t$ thus loosing all the information collected from previous interventions and not accounting for how the previously taken interventions have changed the system.

\textbf{\abo algorithm} \abo addresses dynamic settings but does not account for the causal relationships among variables. As done by \bo, \abo finds the optimal intervention values by breaking the causal dependencies among the inputs and intervening simultaneously on all of them thus setting $\Xst = \Xt$ for all $t$. Additionally, considering the inputs as fixed and not as random variables, \abo does not account for their temporal evolution (see \DAG (c) of \fig \ref{fig:map_methods}). Furthermore, \abo considers a continuous time space and places a surrogate model on $\Yt = f(\x, t)$. Considering a spatio-temporal \gptext allows \abo to predict the objective function ahead in time and track the evolution of the optimum. This is useful when the objective function rate of change over time is slow to gather enough samples to learn the relationships in space and time. In our discrete time setting this condition is equivalent to ask that the objective functions for different interventions do not change overtime. While this can be true in some stationary settings, it might not be the case in non stationary setting where both the \DAG and the \sem evolve overtime. In this settings \abo convergence is significantly slower.  

\our addresses both \cbo and \abo shortcomings. \our considers a different objective function at every time step, incorporates prior interventional information in the objective function and limits the search space at every time step based on the topology of the $\graph$. In addition, through the causal graph, \our imposes additional structure on the surrogate models. This allows \our to better track the dynamic of the objective function and deal with sharp changes in the objectives. \our is thus a framework that can be practically used for sequential decision making in a variety of applications.

\nd{Have to compare and contrast to reinforcement learning.}

==> sections/methodology_model.tex <==
% \input{figures/fig_sections/fig_toy_example}
\subsection{Dynamic Causal \gptext model}
Here we introduce the Dynamic Causal \gptext model that is used as a surrogate model for the objective functions in \cref{eq:dcgo}. The prior parameters are constructed by exploiting the recursion in \eq \eqref{eq: theorem_eq}. At each time step $t$, the agent explores the sets in $\mathbb{M}_t \subseteq \mathcal{P}(\X_t)$ by selecting the next intervention to be the one maximizing a given acquisition function. The \our algorithm is shown in \cref{alg:dcbo_alg}.

\textbf{Prior Surrogate Model}
\label{sec:dc_model}
At each time step $t$ and for each $\Xst \in \missets_t$, we place a \gptext prior on the objective function $\fst(\x) =  \expectation{}{\Yt|\DO{\Xst}{\x}, \mathds{1}_{t>0} \cdot \IPrev}$. We construct the prior parameters exploiting the recursive expression in \cref{eq: theorem_eq}: 
\begin{align*}
 &\fst(\x) \sim \mathcal{GP}(\mst(\x), \kst(\x, \x')) \text{ where } 
 \\
 &\mst(\x) = \expectation{}{\fyy(\vecfopt) +
 \widehat{\mathbb{E}}_{}[\fyny(\apy, \bpy, \w)]} \wedge \kst(\x, \x') = k_{\rbf}(\x, \x') + \sigmast(\x)\sigmast(\x')
\end{align*}
with $\sigmast(\x) = \sqrt{\mathbb{V}[\fyy(\vecfopt) +
\hat{\mathbb{E}}_{}[\fyny(\apy, \bpy, \w)]}$ and $k_{\rbf}(\x, \x') \coloneqq  \exp(-\frac{||\x -\x'||^2}{2l^2})$ represents the radial basis function kernel \cite{rasmussen2003gaussian}. $\hat{\mathbb{E}}_{}[\fyny(\apy, \bpy, \w)] = \hat{\mathbb{E}}_{p(\w|\DO{\Xst}{\x}, \iprev)}[\fyny(\apy, \bpy, \w)]$ represents the expected value of $\fyny(\apy, \bpy, \w)$ with respect to $p(\w \mid \DO{\Xst}{\x}, \iprev)$ which is estimated via the do-calculus using observational data. The outer expectation in $\mst(\x)$ and the variance in $\sigmast(\x)$ are computed with respect to $p(\fyy, \fyny)$ which is also estimated using observational data. In this work we model $\fyy$, $\fyny$ and all functions in the \sem by independent \gptext{s}. 
%However, any alternative probabilistic model can be used.
%to learn these functions. 
%We give estimation details for all experiments in the supplement (\S X). 

Both $\mst(\x)$ and $\sigmast(\x)$ can be equivalently written by exploiting the equivalence in \eq \eqref{eq:alter_expression}. In both cases, this prior construction allows the integration of three different types of data: observational data, interventional data collected at time $t$ and the optimal interventional data points collected in the past. The former is used to estimate the \sem model and $p(\w|\DO{\Xst}{\x}, \iprev)$ via the rules of do-calculus. The optimal interventional data points at $0:t-1$ determine the shift $\fyy(\vecfopt)$ while the interventional data collected at time $t$ are used to update the prior distribution on $\fst(\x)$. Similar prior constructions were previously considered in statistic settings \cite{cbo, daggp} where only observational and interventional data at the current time step were used. The additional shift term appears here as there exists causal dynamics in the target variables and the objective function is affected by previous decisions. \cref{fig:toy_example} in the appendix shows a synthetic example in which accounting for the dynamic aspect in the prior formulation leads to a more accurate \gptext posterior compared to the baselines, especially 
%when the objective function shift due to previous interventions, 
when the the optimum location changes across time steps. 
%(see right panel, 1\textsuperscript{st} and 2\textsuperscript{nd} row). In turns, this lead to a faster convergence of the algorithm to the true optimum (\cref{fig:toy_example} right panel, 3\textsuperscript{rd} row).  

%
\textbf{Likelihood}
Let $\DIntXst = (\DIntXstX, \DIntXstY)$ be the set of interventional datapoints collected for $\Xst$ with $\DIntXstX$ being a vector of intervention values and $\DIntXstY$ representing the corresponding vector of observed target values. As in standard \bo we assume each $\yst$ in $\DIntXstY$ to be a noisy observation of the function $\fst(\x)$ that is $\yst(\x) = \fst(\x) + \epsst$ with $\epsst \sim \normal(0, \sigma^2)$ for $s \in \{1, \dots, |\missets_t|\}$ and $t \in \{0,\dots, T\}$. In compact form, the joint likelihood function for $\DIntXst$ is $p(\DIntXstY \mid \fst, \sigma^2) = \normal(\fst(\DIntXstX),\sigma^2 \mat{I})$. 
%

\textbf{Acquisition Function}
Given our surrogate models at time $t$, the agent selects the interventions to implement by solving a Causal Bayesian Optimization problem \cite{cbo}. The agent explores the sets in $\missets_t$ and decides where to intervene by maximizing the Causal Expected Improvement (\ei). Denote by $\ytstar$ the optimal observed target value in $\{\DIntXstY\}_{s=1}^{|\missets_t|}$ that is the optimal observed target across all intervention sets at time $t$. The Causal \EI is given by $\EIst(\x) = \expectation{p(\yst)}{\text{max}(\yst-\ytstar, 0)}/\texttt{cost}(\Xst, \x_{s,t})$. Let $\alpha_1, \dots, \alpha_{|\missets_t|}$ be solutions of the optimization of $\EIst(\x)$ for each set in $\missets_t$ and $\alpha^\star := \max \{\alpha_1, \dots, \alpha_{|\missets_t|}\}$. The next best intervention to explore at time $t$ is given by $s^\star = \argmax_{s \in \{1, \cdots, |\missets_t|\}} \alpha_s.$ Therefore, the set-value pair to intervene on is $(s^\star, \alpha^\star)$. At every $t$, the agents implement $H$ \emph{explorative} interventions in the system which are selected by maximizing the Causal \ei. 
%At the $p$-th step, $p(\yst)$ in $\EIst(\x)$ will be computed using the the surrogate model updated with the information collected during the $0:p-1$ steps. 
Once the budget $H$ is exhausted, the agent implements what we call the \emph{decision} intervention $I_t$, that is the optimal intervention found at the current time step, and move forward to a new optimization at $t+1$ carrying the information in $\ytotstar$. The parameter $H$ determines the level of exploration of the system and acts as a budget for the \cbo algorithm. Its value is determined by the agent and is generally problem specific. 
% For instance, consider the air pollution example mentioned in Section X. Local administrations might be allowed to change the implemented policy every year thus the time index $t$ might correspond to the year index. However, within a certain year, they can perform \emph{explorative interventions} allowing them to collect information about the variable they are trying to optimize and the causal effect of different interventions. The Dynamic Causal \gptext model allows them to integrate all the collected information in a principled way.
%
% Based on the optimal intervention identified during the trial phase, local administrations can then implement a \emph{decision} intervention that will permanently change the system and, by propagating in the system, will affect its future state and the future decisions. 
%
%Note that $P$ trials might not be enough to find the true optimal interventions at time $t$. However, this will be the intervention propagated in the system that will determine the target function to optimize at $t+1$ and the target value we can reach at subsequent time steps (see \fig X).
%

\textbf{Posterior Surrogate Model}
For any set $\Xst \in \missets_t$, the posterior distribution $p(\fst \mid \DIntXst)$ can be derived analytically via standard \gptext updates. $p(\fst|\DIntXst)$ will also be a \gptext with parameters $\mst(\x \mid \DIntXst) = \mst(\x) + \kst(\x, \DIntXstX)[\kst(\DIntXstX, \DIntXstX) + \sigma^2\mat{I}])(\DIntXstY - \mst(\DIntXstX)$ and $\kst(\x, \x' \mid \DIntXst)= \kst(\x, \x') - \kst(\x, \DIntXstX)[\kst(\DIntXstX, \DIntXstX) + \sigma^2\mat{I}])\kst(\DIntXstX, \x')$.
% We give the complete \our algorithm in \cref{alg:dcbo_alg}. The time complexity of \dcbo is dominated by algebraic operations on $\kst(\DIntXstX, \DIntXstX)$ which are $\mathcal{O}(P^3)$ where $P$ denotes the number of collected interventional data points. The space complexity is $\mathcal{O}(P^2)$. 
%
%This posterior is used to form the acquisition function α(x, Dn), which can be chosen among popular acquisition functions such as expected improvement or entropy search. The next evaluation is placed at the (numerically estimated) global maximum of α(x, Dn).
%The optimization problem we solve at time $t$ can be seen as a local optimization of the objective function with respect to the $t$-dimension. Instead of searching for the optimal intervention maximizing $Y_T$ in $\graph_{0:T}$, we solve local optimization along one dimension of the function. See Fig 1 for a graphical representation of what the method is doing in \DAG X.
%looking for the global maximum of $Y_T$ and having as action space the all the possible interventions in the graph we do local optimization along one dimension of the function.
%There are two important things to notice here. First of all, the solution found at time $t$ might not be the true optimal interventions as the $P$ trials were not enough to find it. This is gonna determined the target function we optimize at $t+1$ and the target value we can reach.  
% the value that do not overlap are due to the fact that that is the true otpimal function we can target at t+1, it is not wrong, the other function is just not recheable anymore. 
% Notice that in \our only the intervention decision affects the prior on the target function at $t+1$ via the term $\fyy(\vecfopt)$. The information obtained from the explorative interventions is disregarded in surrogate model. In order to avoid this, one would need to modify the Dynamic Causal \gptext{s} to have a joint model across different intervention sets and different intervention values. We leave this for future research. 

% The joint model would capture the correlation both between $\fst$ and $f_{s', t}$ and across the values of $\fst$ computed in different $\IPrev$. 
%Finally, notice that the transfer of information from $t-1$ to $t$ is affected by the accuracy of the estimation of the functions in the \sem. The more accurate these estimations are, the closer the mean function $\mst(\x)$ is to the true objective function. Higher accuracy also leads to lower $\sigmast(\x)$ and thus lower uncertainty around the true function. On the contrary, lower accuracy inflates the variance on $\fst$ making \our robust to poor estimation of the \sem.

% \subsection{The \our algorithm}
% \label{sec:alg_section}

% We give the complete \our algorithm in \cref{alg:dcbo_alg}. The time complexity of \our is dominated by algebraic operations on $\kst(\x, \x')$ which are $\mathcal{O}(P^3)$ where $P$ denotes the number of function evaluations of the \bo algorithm at every time step. The space complexity is dominated by storing $\kst(\x, \x')$ which is $\mathcal{O}(P^2)$.

\begin{wrapfigure}{R}{0.45\textwidth}
    \vspace{-5em}
    \begin{minipage}{.5\textwidth}
    \scalebox{0.90}{
        \begin{algorithm}[H]
        	\SetKwInOut{Input}{input}
        	\SetKwInOut{Output}{output}
        	\KwData{$\dataset^O$, $\{\DIntXstzero\}_{s \in \{0,\dots, |\missets_0|\}}$, $\graph_{0:T}$, 
        	$H$. }
        	\KwResult{Optimal intervention path $\{\Xst^\star, \xst^\star, y_t^\star\}_{t = 1}^T$}
        	\textbf{Initialise}: $\missets$, $\dataset^I_0$ and initial optimal $\DIopt = \emptyset$.\\
        	\For{$t = 0, \dots, T$}{ 
        	1. Initialise dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\mathcal{D}^I_{\star,t-1}$ if $t>0$. \\
        	2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$ \\
        	\For{$h = 1, \dots, H$}{
        	1. Compute $\EIst(\x)$ for each $\Xst \in \missets_t$.\\
        	2. Obtain $(s^\star, \alpha^\star)$ \\
        	3. Intervene and augment $\DIntXsstar$ \\
        	4. Update posterior for $f_{s=s^\star, t}$
            }
            3. Return the optimal intervention $(\Xst^\star, \xst^\star)$\\
            4. Append optimal interventional data $\mathcal{D}^I_{\star,t} = \mathcal{D}^I_{\star,t-1} \cup ((\Xst^\star, \xst^\star), y^\star_t)$
        	}
        	\caption{\our}
        	\label{alg:dcbo_alg}
        \end{algorithm}
    }
    \end{minipage}
    \vspace{-1em}
\end{wrapfigure}


% \virgi{don't check the remaining of this section}

% \paragraph{Detecting non-stationarity} Non-stationary distributions manifests themselves in our setting in two ways: (1) through the CGM or (2) through the SEM. In the former case it is clear that given a non-constant topological structure across time, gives rise to non-stationary behaviour in the observations governed by this topology. However, it is still possible to observe non-stationary behaviour even if the graph topology is constant across time. In this case the non-stationarity will originate in the SEM. Hence, in the first case it is simple enough to detect non-stationarity, since in this work we assume we know the CGM, but in the second case it becomes more difficult, if we are using real observational data. Consequently we need to determine if the observational distribution has shifted substantially between time-steps, so much so that the change gives rise to non-stationary statistics. 

% In this work we are using Gaussian processes as our method of choice for estimating the causal effects in the CGM. Owing to this we will consider similarity measures between GPs in order to detect non-stationarity. This being said, there is a rich literature on non-stationary detection as well, \nd{CPD, HMM, KS tests, Lee-Addler tests, WD and so on} and many of those methods would be suitable here too. 


% \nd{We don't really need most of this section, just the algorithm.}

% \input{sections/alg}



==> sections/methodology_search_space.tex <==
\subsection{Restricting the search space}
\label{sec:space}
The search space for the problem in \cref{eq:dcgo} grows exponentially with $|\mat{X}_t|$ thus slowing down the identification of the optimal intervention when $\graph$ includes more than a few nodes. Indeed, a naive approach to find $\mat{X}_{s,t}^\star$ at $t=0, \dots, T$ would be to explore the $2^{|\mat{X}_t|}$ sets in $\mathcal{P}(\mat{X}_t)$ at every $t$ and keep $2^{|\mat{X}_t|}$ models for the objective functions. In the static setting, \cbo reduces the search space by exploiting invariances in the interventional space \cite{lee2018structural} to identify a subset of intervention sets $\missets \subseteq \mathcal{P}(\X)$ worth exploring. 
% Exploiting the rules of do-calculus, \citet{lee2018structural} identify invariances in the interventional space that can be exploited the reduce the dimensionality of the search space in the static \cbo setting. These results have been used in \cbo to reduce the search space to a subset $\missets$ ES of the power. with each sey in being a  set of variables that is worth intervening on. 
% They define the minimal intervention sets as follow:
% \begin{definition}{\textbf{Minimal Intervention set (\mis).}}
% Given $\langle \graph, \mat{Y}, \mat{X},\mat{C} \rangle$, a set of variables $\mat{X}_s \in \mathcal{P}(\mat{X})$ is said to be a \mis if there is no $\mat{X}'_s \subset \mat{X}_s$ such that $\expectation{}{Y| \DO{\mat{X}_s }{\x_s}} = \expectation{}{Y|\DO{\mat{X}'_s }{\x'_s}}$. 
% \end{definition}
% Denote by $\missets$ the set of \mis{s} for $\langle \graph, \mat{Y}, \mat{X},\mat{C} \rangle$ where each \mis represents a set of variables that is worth intervening on. 
In our dynamic setting, the objective functions change at every time step depending on the previously implemented interventions and one would need to recompute $\missets$ at every $t$. However, it is possible to show that, given Assumptions (\ref{assumptions}), the search space remains constant over time. Denote by $\missets_t$ the set $\missets$ at time $t$ and let $\missets_0$ represent the set at $t=0$ which corresponds to $\missets$ computed in \cbo. For $t>0$ it is possible to prove that: 
\begin{proposition}{\textbf{\mis in time.}} If Assumptions (\ref{assumptions}) are satisfied, $\mathbb{M}_t = \mathbb{M}_0$ for $t>0$.
\end{proposition}
%(see proof in Section X of the supplement)
% For each set $\mat{X}_s \in \mathcal{P}(\mat{X})$ that is not a \mis set, we call $\Ss = \mat{X}_s \backslash \mat{X}'_s $ the set of \emph{superfluous} variables that are those variables not needed in the computation of the objective function. 
% We denote by $\missets$ the set of \mis{s} for $\langle \graph, \mat{Y}, \mat{X},\mat{C} \rangle$ where each \mis represents a set of variables that is worth intervening on. On the contrary, $\Sset = \mathcal{P}(\mat{X}) \backslash \missets$ represents the non \mis sets that should not be explored by the optimization algorithm. In our dynamic optimization setting, the objective functions change at every time step depending on the previously implemented interventions. As a consequence, one would need to recompute $\missets$ in order to identify the intervention sets worth exploring at every $t$. However, it is possible to show that, given Assumptions (\ref{assumptions}), the search space remains constant over time. In other words, the same intervention sets need to be explored at every time step. Denote $\missets$ at time $t$ by $\missets_t$ and let $\missets_0$ represent the set of \mis{s} at $t=0$ which corresponds to $\missets$ computed in \cbo. For $t>0$ we have the following (see proof in Section X of the supplement): 

% \begin{proposition}{\textbf{\mis in time.}} If Assumptions (\ref{assumptions}) are satisfied, $\mathbb{M}_t = \mathbb{M}_0$ for $t>0$.
% \end{proposition}

%\vspace{-0.4cm}

==> sections/related_work.tex <==
\subsection{Related Work}
\label{sec:related_work}

\nd{Have not touched this section yet.

% Optimization in dynamic settings
\textbf{Dynamic Optimization} Optimization in dynamic environments has studied in the context of evolutionary algorithms \cite{fogel1966artificial, goldberg1987nonstationary}. More recently, other optimization techniques \cite{pelta2009simple, trojanowski2009immune, de2006stochastic} have been adapted to dynamic settings, see e.g. \cite{cruz2011optimization} for a review. Focusing on \bo, the literature on dynamic settings \cite{azimi2011dynamic, bogunovic2016time, abo} is limited. 
% \citet{azimi2011dynamic} performed batch \bo in a dynamic setting where the batch sizes are dynamically determined. \citet{bogunovic2016time} introduced a \bo algorithm with bandit feedback and a reward function that varies with time. More recently, \citet{abo} developed \abo, a framework for solving \bo on continuous spaces when the function evolution follows a more complex behaviour than a simple Markov model. 
The dynamic \bo framework closest to this work is given by \citet{abo} and focuses on functions defined on continuous spaces that follow a more complex behaviour than a simple Markov model. \abo treats the inputs as fixed and not as random variables, thereby disregarding their temporal evolution and, more importantly, breaking their causal dependencies. 
% In addition, \abo requires a slow rate of change of the objective function so as to gather enough samples to learn the function evolution over space and time. All these methods tackle the dynamic dimension of the problems we address but do not account for the causal relationships among variables. 

% Causal Optimization
\textbf{Causal Optimization} Causal \bo \citep[\cbo,][]{cbo} focuses instead on the causal aspect of optimization and solves the problem of finding an optimal intervention in a \DAG by modelling the intervention functions with single \gptext{s} or a multi-task \gptext model \cite{daggp}. \cbo disregards the existence of a temporal evolution in both the inputs and the output variable, treating them as \iid overtime. While disregarding time significantly simplifies the problem, it prevents the identification of an optimal intervention at every $t$. 
%In many practical applications, the \iid assumption does not provide an adequate description for the data. Indeed, different causal methodologies %and extensions of structural causal models have been adapted to deal with longitudinal studies \cite{granger1969investigating, white2010granger, peters2012causal, hyttinen2013discovering, pfister2019invariant}. See \cite{peters2009detecting,bauer2016arrow} for a discussion of the relation between causality and the arrow of time. 

\textbf{Bandits and \rl} In the broader decision-making literature, causal relationships have been considered in the context of bandits \citep{bareinboim2015bandits, lattimore2016causal, lee2018structural, lee2019structural} and reinforcement learning \citep{lu2018deconfounding, buesing2018woulda, foerster2018counterfactual, zhang2019near, madumal2020explainable}. In these cases, actions or arms, correspond to interventions on a causal graph where there exists complex links between the agent’s decisions and the received rewards. While dynamic settings have been considered in acausal bandit algorithms \citep{besbes2014stochastic, villar2015multi, wu2018learning}, causal \mab have focused on static settings.  
Dynamic settings are instead considered by \rl algorithms and formalized through Markov decision processes (\acro{mdp}). In the current formulation, \our does not consider a \acro{mdp} as we do not have a notion of \emph{state} and therefore do not require an explicit model of its dynamics. The system is fully specified by the causal model. As in \bo, we focus on identifying a set of time-indexed optimal actions rather than an optimal policy. We allow the agent to perform explorative interventions that do not lead to state transitions. More importantly, differently from both \mab and \rl, \emph{we allow for the integration of both observational and interventional data}. 
An expanded discussion on the reason why \our should be used and the links between \our, \cbo, \abo and \rl is included in the appendix (\cref{sec:connections}). 
% that generally focus on learning an optimal policy by accounting for non stationaruty in the rewards. 
% Differenlty from \rl, \our identifies a set of optimal actions as in \bo. In \our does not have a notion of \emph{state} and therefore does not require an explicit model of its dynamic which is fully specified by the causal graph and the structural equation model. 
}
% %%%

% Instead, \rl algorithms explicitly model the state dynamic and let every action affect the environment\theo{is it the environment or the state of the agent?(which is a state of the environment but depends on your notion of agent and environment)}. Conversely, \our does not have a notion of \emph{state} and therefore does not require an explicit model of its dynamic which is fully specified by the causal graph and the structural equation model. Finally, while \rl aims at learning an optimal policy \theo{not necessarily - can also aim to evaluate a given policy right?}, \our identifies a set of optimal actions as in \bo. 



==> sections/table_sections/table_metric_perc.tex <==
\begin{table}
% \vspace{-1.5em}
\centering
\caption{Average \% of replicates across time steps for which $\Xst^\star$ is identified. See \cref{fig:map_methods} for a summary of the baselines. Higher values are better. The best result for each experiment in bold. }
\label{tab:table_sets}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
&  \multicolumn{6}{c}{Synthetic data} & \multicolumn{2}{c}{Real data} \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
& \expone & \expmissing & \expnoise &  \expcomplex & \expindep & \expnonstat & \exprealec & \exprealpol \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
\multirow{1}{*}{$\our$} & \textbf{93.00} & 58.00 & \textbf{100.00} & \textbf{93.00} & 93.00 & \textbf{100.00} & 86.67 & \textbf{33.3}\\
\multirow{1}{*}{$\cbo$} & 90.00 & \textbf{85.00} & 90.00 & 90.0 & 90.00 & \textbf{100.00} & \textbf{93.33} & \textbf{33.3}\\
\multirow{1}{*}{$\abo$} & 0.00 & 0.00 & 0.00 & 0.00 & \textbf{100.00} & 0.00 & 66.67 & 0.00 \\
\multirow{1}{*}{$\bo$} & 0.00 & 0.00 & 0.00 & 0.00 & \textbf{100.00} & 0.00 & 66.67 & 0.00 \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
\end{table}

==> sections/table_sections/table_metrics.tex <==
\begin{table}[hb!]
\vspace{-1em}
\centering
\caption{Average $\gap_t$ across 10 replicates and time steps. See \cref{fig:map_methods} for a summary of the baselines. Higher values are better. The best result for each experiment in bold. Standard errors in brackets. }
\label{tab:table_gaps}
\resizebox{\columnwidth}{!}{
%@{\extracolsep{4pt}}@{\kern\tabcolsep}
\begin{tabular}{lcccccccc}
\toprule
&  \multicolumn{6}{c}{Synthetic data} & \multicolumn{2}{c}{Real data} \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
& \expone & \expmissing & \expnoise &  \expcomplex & \expindep & \expnonstat & \exprealec & \exprealpol \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
\multirow{2}{*}{$\our$} & \textbf{0.88}   &  \textbf{0.84} & \textbf{0.75} & \textbf{0.49} & 0.48 & \textbf{0.69}  & \textbf{0.64} & \textbf{0.67}  \\
          & (0.00) & (0.01)  & (0.00) & (0.01) & (0.04) & (0.00) & (0.01) & (0.00)\\
\multirow{2}{*}{$\cbo$} & 0.70  & 0.70 &  0.51  & 0.48 & 0.47  & 0.61 & 0.61 & 0.65\\
          & (0.01) & (0.02) & (0.02) & (0.09) & (0.07) & (0.00) & (0.01) & (0.00)\\
\multirow{2}{*}{$\abo$} & 0.56  & 0.49 & 0.49 & 0.39 & \textbf{0.54} & 0.38 & 0.57  & 0.48\\
          & (0.01) & (0.02) & (0.04) & (0.21) & (0.01) & (0.02) & (0.02) & (0.01)\\
\multirow{2}{*}{$\bo$} & 0.54  & 0.48 & 0.38 & 0.35 & 0.50 & 0.38 & 0.50 & 0.44\\
          & (0.02) & (0.03) & (0.05) & (0.08) & (0.01) & (0.03) & (0.01) & (0.03)\\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table}



==> sections/table_sections/table_no_convergence.tex <==
\begin{table}[htbp]
\centering
\caption{Average modified gap measure (10 replicates) across time steps and for different experiments. See \fig \ref{fig:map_methods} for a summary of the compared methods. Higher values are better. The best result for each experiment is bolded. Standard errors in brackets.}
\label{tab:table_gaps_noconv}
\resizebox{\columnwidth}{!}{
%@{\extracolsep{4pt}}@{\kern\tabcolsep}
\begin{tabular}{lcccccccc}
\toprule
&  \multicolumn{6}{c}{Synthetic data} & \multicolumn{2}{c}{Real data} \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
& \expone & \expmissing & \expnoise &  \expcomplex & \expindep & \expnonstat & \exprealec & \exprealpol \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
\multirow{2}{*}{$\our$} &  \textbf{0.88} & \textbf{0.72}  & \textbf{0.73} & \textbf{0.49} & 0.47 & \textbf{0.47} & 0.40 &  \textbf{0.67}\\
          &  (0.00) & (0.07) & (0.00) & (0.00) & (0.05) & (0.00) & (0.04) & (0.00) \\
\multirow{2}{*}{$\cbo$} & 0.57 & 0.51 & 0.67 & 0.47 & 0.48 & \textbf{0.47} & \textbf{0.41} & 0.65 \\
          & (0.02) & (0.09) & (0.01) & (0.04) & (0.04) & (0.00) & (0.04) & (0.00)\\
\multirow{2}{*}{$\abo$} & 0.43 & 0.45 & 0.42 & 0.40 & \textbf{0.50} & 0.41 & 0.38 & 0.47\\
          & (0.06) & (0.04) & (0.06) & (0.05) & (0.00) & (0.03) & (0.04) & (0.01) \\
\multirow{2}{*}{$\bo$} & 0.42 & 0.41 & 0.41 & 0.38 & \textbf{0.50} & 0.40& 0.40 & 0.46\\
          & (0.06) & (0.05) & (0.07) & (0.07) & (0.01) & (0.04) & (0.04) & (0.03)\\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[htbp]
\centering
\caption{Average percentage of replicates across time steps and for different experiments for which the optimal intervention set is identified. See \fig \ref{fig:map_methods} for a summary of the compared methods. Higher values are better. The best result for each experiment is bolded.}
\label{tab:table_sets_noconv}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
&  \multicolumn{6}{c}{Synthetic data} & \multicolumn{2}{c}{Real data} \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
& \expone & \expmissing & \expnoise &  \expcomplex & \expindep & \expnonstat & \exprealec & \exprealpol \\
\cmidrule(lr){2-7} 
\cmidrule(lr){8-9}
\multirow{1}{*}{$\our$} & \textbf{90.0} & \textbf{70.00} & \textbf{93.00}  & \textbf{93.33} & \textbf{96.67} & \textbf{66.67} & 73.33 & \textbf{33.33} \\
\multirow{1}{*}{$\cbo$} & 76.67 & 63.33 & 76.67 & 86.67 & 93.33 & 33.33 &   \textbf{80.00} & \textbf{33.33}\\
\multirow{1}{*}{$\abo$} & 0.00 & 0.00 & 0.00 & 0.00 & 100.00 & 0.00 & 66.67 & 0.00\\
\multirow{1}{*}{$\bo$} & 0.00 & 0.00 & 0.00 & 0.00 & 100.00 & 0.00 & 66.67 & 0.00\\
\bottomrule
\end{tabular}
}
\end{table}

==> sections/table_sections/table_notation.tex <==
\begin{table}[htbp]
% \caption{Summary of notation used in the paper.}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
% \resizebox{\columnwidth}{!}{
% \setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{tabular}{ccl}
% \toprule
\textbf{Symbol} &  & \textbf{Description} \\
% \toprule
 & & \\
$\mat{V}_{t}$ & & Set of observable variables at time $t$ \\
$\mat{V}_{0:T}$ & & Union of observable variables at time $t = 0,\dots, T$  \\
$\mat{X}_t$ & & Manipulative variables at time $t$ \\
$Y_t$ & & Target variable at time $t$ \\
$\mathcal{P}(\mat{X}_t)$ &  & Power set of $\mat{X}_t$ \\
$\mathbb{M}_t$ &  & Set of \mis sets at time $t$   \\
$\mat{X}_{s,t}$ &  & $s$-th intervention set at time $t$ \\
$\dataset$ &  & Observational dataset $\{\mat{V}^i_{0:T}\}_{i=1}^N$\\
$N$ &  &  Number of observational data points collected from the system \\
$\DIntXst$ &  & Interventional data points  collected for the intervention set $\Xst$\\
$\DIntXstX$ & & Vector of interventional values \\
$\DIntXstY$ & & Vector of target values obtained by intervening on $\Xst$ at $\DIntXstX$ \\
$H$ &  &  Maximum number of explorative interventions an agent can conduct at every $t$ \\
$I_{0:t-1}$ & & Decision Interventions at time step $0$ to $t-1$\\
$\fst$ &  & Objective function for the set $\Xst$
\\
$\mst$ &  & Prior mean function of \gptext on $\fst$
\\
$\kst$ &  & Prior kernel function of \gptext on $\fst$ \\
$\mst(\cdot\mid \DIntXst)$ &  & Posterior mean function for \gptext on $\fst$ \\
$\kst(\cdot, \cdot\mid\DIntXst)$ &  & Posterior covariance function for \gptext on $\fst$ 
\\
% \bottomrule
\end{tabular}
% }
\end{center}
\label{tab:TableOfNotation}
\end{table}


==> sections/table_sections/table_plankton.tex <==
\begin{table}[htbp]
\centering
\caption{Table describing variable and parameters of ODE in \cref{eq:ode_N} -- \cref{eq:ode_D}.\label{table:ode}}
\begin{tabular}{clcc}
\toprule
Variable & Description & Value & Unit \\
\midrule
$N$ & Nitrogen (prey) concentration & $\in \mathbb{R}^1$ & $\unit$ \\ 
$P$ & Phytoplankton (predator) concentration & $\in \mathbb{R}^1$ & $\unit$ \\ 
$E$ & Predator egg concentration & $\in \mathbb{R}^1$ & $\unit$ \\ 
$J$ & Predator juvenile concentration & $\in \mathbb{R}^1$ & $\unit$ \\ 
$A$ & Predator adult concentration & $\in \mathbb{R}^1$ & $\unit$ \\ 
$D$ & Dead animal concentration & $\in \mathbb{R}^1$ & $\unit$ \\
\midrule
Parameter & Description & Value & Unit \\
\midrule
$N_{\text{in}}$ & Nitrogen concentration in the external medium & 80 & $\unit$ \\
$F_P$ & Algal nutrient uptake & - & $\unit$ \\
$F_B$ & Rotifer nutrient uptake & - & $\unit$\\
$\varepsilon$ & Predator assimilation efficiency & 0.55 & - \\
$R_E$ & Egg recruitment rate & - & -\\
$R_J$ & Juvenile recruitment rate & - & -\\
$R_A$ & Adult recruitment rate & - & -\\
$m$ & Rotifer (predator) mortality rate & 0.15 & Per day\\
$\beta$ & Adult/juvenile mass ratio & 5 & - \\
\bottomrule
\end{tabular}
\end{table}
